An Efficient Algorithm to Calculate BICM Capacity

Bit-interleaved coded modulation (BICM) is a practical approach for reliable communication over the AWGN channel in the bandwidth limited regime. For a signal point constellation with 2^m points, BICM labels the signal points with bit strings of length m and then treats these m bits separately both at the transmitter and the receiver. BICM capacity is defined as the maximum of a certain achievable rate. Maximization has to be done over the probability mass functions (pmf) of the bits. This is a non-convex optimization problem. So far, the optimal bit pmfs were determined via exhaustive search, which is of exponential complexity in m. In this work, an algorithm called bit-alternating convex concave method (Bacm) is developed. This algorithm calculates BICM capacity with a complexity that scales approximately as m^3. The algorithm iteratively applies convex optimization techniques. Bacm is used to calculate BICM capacity of 4,8,16,32, and 64-PAM in AWGN. For PAM constellations with more than 8 points, the presented values are the first results known in the literature.

==> Makefile <==
PROJECT=bacm
TMPFILES=*.aux *.bak *.bbl *.blg *.lof *.log *.toc *.lot *~ *.backup\
*.pfx *.ovp $(PROJECT)-pics.* $(PROJECT).dvi $(PROJECT).ps\
*.ind *.idx *.ilg *.gls *.glo *.glg *.acn *.acr *.alg *.ist *.out\
*.thm
ARXIVTMP=*.aux *.bak *.blg *.lof *.log *.toc *.lot *~ *.backup\
*.pfx *.ovp $(PROJECT)-pics.* $(PROJECT).dvi $(PROJECT).ps $(PROJECT).pdf *.bib .*.xml


default:
	pdflatex $(PROJECT).tex;

clean:
	rm -f $(TMPFILES);

clean_pdf:
	rm -f $(PROJECT).pdf;

final: clean clean_pdf
	pdflatex -shell-escape $(PROJECT).tex;
	pdflatex $(PROJECT).tex;
	bibtex $(PROJECT);
	pdflatex $(PROJECT).tex;
	pdflatex $(PROJECT).tex;
	pdflatex $(PROJECT).tex;
arxiv:
	rm -f $(ARXIVTMP);
	rm -rf .git;



==> conclusions.tex <==
\section{Conclusions}
\label{sec:conclusions}
In this work, we made a first step towards efficiently calculating BICM capacity using iterative techniques from convex optimization. The complexity of our algorithm increases linearly with the number of bit positions $m$ of the input, opposed to exhaustive search, whose complexity increases exponentially in $m$. Given a good starting point, our algorithm finds BICM capacity of DMCs. Furthermore, for a cost vector $\vecw$ and a Lagrange multiplier $\lambda$, BACM finds optimal points on the BICM capacity-cost curve. Using our algorithm, we were able to calculate for the first time the BICM capacity-cost function of 16 PAM in AWGN. For future research, it would be nice to find a method that can calculate BICM capacity for a given power constraint $E$.


==> numerical.tex <==
\section{Application to PAM in AWGN}
\begin{figure}
\footnotesize
\def\svgwidth{\columnwidth}
\includesvg{figures/bicmmi-edited}
\caption{For $m=2,3,4,5,6$ we calculate the maximum BICM mutual information for $2^m$-PAM in AWGN.}
\label{fig:awgn}
\end{figure}
We use our algorithm \textsc{Bacm} to calculate the BICM capacity of equidistant PAM constellations in AWGN. The input signal points are labelled according to a binary reflected Gray code (BRGC). The parameters over which we have to optimize is the scaling of the constellation and the bit pmfs. This optimization has to be done subject to a power constraint that corresponds to the SNR value of interest. Our approach to solve this problem is as follows.
\begin{itemize}
\item For a given value $\gamma$ of the scaling and $M=2^m$, the constellation is
\begin{align}
\mathcal{X}=\gamma\cdot\{-M+1,-M-1,\dotsc,M-3,M-1\}.
\end{align}
We index the signal points in $\mathcal{X}$ according to the BRGC labeling, i.e., such that \eqref{eq:labeling} holds. Each input symbol $x_i\in\mathcal{X}$ has now an associated power given by $w_i=|x_i|^2$.
\item The channel is now given by
\begin{align}
Y=X+Z
\end{align}
where $X$ takes values in $\mathcal{X}$ and where $Z$ is distributed according to a normal distribution, i.e., $Z\sim\mathcal{N}(0,1)$.
\item We discretize the channel output $Y$ into $200$ equally spaced points in an interval $\mathcal{I}$. We choose the interval such that the conditioned output is in this interval with high probability, i.e., for each $x\in\mathcal{X}$, $\probop(Y\in\mathcal{I}|X=x)\approx 1$.
\item The channel can now be characterized by a matrix of transition probabilities $\mathh\in\setr^{200\times M}$.
\end{itemize}
This casts the problem of finding the BICM capacity of an AWGN channel into the problem of finding the BICM capacity of a dmc subject to a cost constraint. We define the $\mathsf{snr}$ as
\begin{align}
\mathsf{snr}=\frac{\expop(|X|^2)}{\expop(|Z|^2)}=\expop(|X|^2).
\end{align}
Since we are interested in bicm capacity, $\expop(|X|^2)$ is given by
\begin{align}
\expop(|X|^2)=\vecw^T(\vecp^1\otimes\dotsb\otimes\vecp^m)
\end{align}
where $\vecp^i$ are the bit pmfs of the signal point labels. Using the technique suggested in Sec.~\ref{sec:power}, we solve
\begin{align}
\maximize_{\vecp^1,\dotsc,\vecp^m}\quad&\bicmmi(\vecp^1,\dotsc,\vecp^m)-\lambda\vecw^T(\vecp^1\otimes\dotsb\otimes\vecp^m)
\end{align}
using the \textsc{Bacm} algorithm. We determine the optimal pmfs with a precision of $d=10^{-5}$. Denote by $\vecp^{*1},\dotsc,\vecp^{*m}$ the optimal pmf of this problem. Define
\begin{align}
\capacity_{\gamma,\lambda}:=\bicmmi(\vecp^{*1},\dotsc,\vecp^{*m}).
\end{align}
BICM capacity for a given value of $\mathsf{snr}$ can now be calculated as follows:
\begin{itemize}
\item For each $\gamma$, choose $\lambda$ such that
\begin{align}
\vecw^T(\vecp^{*1},\dotsc,\vecp^{*m})=\mathsf{snr}.
\end{align}
This can be done via bisection over $\lambda$. Denote the corresponding value of $\bicmmi$ by $\capacity_\gamma(\mathsf{snr})$.
\item Among all values of $\gamma$, choose the one that results in the largest value of $\capacity_\gamma(\mathsf{snr})$. We do this via line search. Declare this largest value of $\capacity_\gamma(\mathsf{snr})$ the BICM capacity $\capacity^\mathrm{bicm}(\mathsf{snr})$.
\end{itemize}
BICM capacity $\capacity^\mathrm{bicm}(\mathsf{snr})$ is bounded from above by the coded modulation capacity, i.e., the greatest mutual information that can be achieved by an $M$-PAM constellation for a given value of $\mathsf{snr}$, where maximization is over all input pmfs and all constellation scalings. BICM capacity is lower bounded by $\bicmmi(\vecu^1,\dotsc,\vecu^m)$, i.e., the BICM mutual information that is achieved if all bit pmfs are uniform. Note that when the pmfs are restricted to be uniform, the value of $\mathsf{snr}$ directly determines the corresponding constellation scaling. We show numerical results for $m=2,3,4,5,6$ in Fig.~\ref{fig:awgn}. For each $m$, we display as a line values we calculated for $\bicmmi$ and display for the target value of $\mathsf{snr}$ the corresponding values for the upper bound $\capacity^\mathrm{cm}(\mathsf{snr})$ and $\capacity^\mathrm{bicm}_\mathrm{u}(\mathsf{snr})$. For all values, the gap in percent to the AWGN capacity $0.5\log(1+\mathsf{snr})$ is displayed. For $4$-PAM, $\bicmmi$ almost hits its upper bound $\capacity^\mathrm{cm}$. For $8$-PAM, the value of $\bicmmi$ at $11$dB corresponds to the value in \cite[Fig.~3.4]{Alvarado2010}, which was found via exhaustive search. For $16$, $32$, and $64$ PAM, no values for comparison are available from the literature. However, at the correesponding values for the target values of $\mathsf{snr}$, the relation between $\capacity^\mathrm{cm}$, $\capacity^\mathrm{bicm}$, and $\capacity_\mathrm{u}^\mathrm{bicm}$ appears similar to the one for $8$ PAM. Furthermore, at all target $\mathsf{snr}$ values, $\capacity^\mathrm{bicm}$ is within $2--3$ percent of AWGN capacity and significantly outperforms $\capacity_\mathrm{u}^\mathrm{bicm}$.





==> outline.tex <==
\section{Our Approach and Main Result}

The objective function $f_0$ is a non-convex function of the probabilities $p^1_0,\dotsc,p^m_0$ with potentially more than one local maxima. Thus, finding an efficient algorithm that provably finds the global maximum is difficult. Therefore, we resort to the simpler problem of finding a local maximum. With a good starting point, the global maximum is nevertheless found by such an approach. To find local maxima, efficient methods are available. For the problem at hand, we choose the combination of two methods.
\begin{itemize}
\item We maximize over one bit pmf $\vecp^i$ at a time and then cycle through the $i=1,\dotsc,m$ until convergence. This approach goes under the name \emph{alternating maximization}.
\item To maximize over one bit pmf, we iteratively approximate the objective function by a concave lower bound and maximize this concave lower bound by convex optimization techniques. Since, as we will see, $\bicmmi$ can be written as the sum of concave and convex functions, this can be done by using the \emph{convex-concave procedure}. After convergence, the maximum of the concave lower bound is also a local maximum of the non-concave objective function $\bicmmi$.
\end{itemize}
We call this approach the \emph{bit-alternating convex-concave method} (\textsc{Bacm}). We show that the complexity of \textsc{Bacm} increases as $m^2$ in the number of bit positions $m$ and as $\log_2\frac{d}{2}$ in the precision $d$. This improves significantly upon exhaustive search, whose complexity increases exponentially in $m$ and polynomially in $d$.

